Near-Optimal Wafer-Scale Reduce

Efficient Reduce and AllReduce communication collectives are a critical cornerstone of high-performance computing (HPC) applications. We present the first systematic investigation of Reduce and AllReduce on the Cerebras Wafer-Scale Engine (WSE). This architecture has been shown to achieve unprecedented performance both for machine learning workloads and other computational problems like FFT. We introduce a performance model to estimate the execution time of algorithms on the WSE and validate our predictions experimentally for a wide range of input sizes. In addition to existing implementations, we design and implement several new algorithms specifically tailored to the architecture. Moreover, we establish a lower bound for the runtime of a Reduce operation on the WSE. Based on our model, we automatically generate code that achieves near-optimal performance across the whole range of input sizes. Experiments demonstrate that our new Reduce and AllReduce algorithms outperform the current vendor solution by up to 3.27x. Additionally, our model predicts performance with less than 4% error. The proposed communication collectives increase the range of HPC applications that can benefit from the high throughput of the WSE. Our model-driven methodology demonstrates a disciplined approach that can lead the way to further algorithmic advancements on wafer-scale architectures.

==> results.tex <==
\section{Experiments}\label{sec:experiments}
We evaluate the performance of different collectives for a row of PEs as well as a square grid of PEs. For each of the collective, we perform two types of experiments. All data types are 32-bit floating point numbers. In the first experiment type, we fix the number of PEs $P$ to be the maximum row length or grid size that is still a power of two and vary the vector length $B$. A large grid size caters to the fact that HPC applications need to utilize most of the PEs to achieve the best performance. The second experiment type fixes the vector length $B$ to 256 values (1 KB) and varies the number of PEs in a row or grid. This allows us to see how performance and our predictions are impacted by the number of PEs.

% . We discuss how well our model's predictions compare against the hardware measurements


% Experimental Setup
\subsection{Benchmarking} All benchmarks are on a CS-2 running at 850 MHz with $40$GB of on-chip SRAM. % and a peak on-chip memory bandwith of X GB/s. % Variance
We run each benchmark $5$ times and plot the mean runtime. The observed standard deviation is negligible (<~4\%)~\cite{scbench}. Five measurements is enough because the CS-2 is mostly deterministic unlike traditional architectures. There is no caching and memory access time is deterministic. The time to travel between the routers is also always 1 cycle. One source of non-determinism is that PEs may insert no-ops to regulate thermal stress of the wafer. Additionally, although the cores all run at around 850 MHz, they are truly independent cores, with independent clocks. For these reasons we still see some deviation from the mean. The performance will also depend the specific CS-2 chip. If there are any defects, a proprietary process will route around them. %, although in the worst case it is $31$ cycles.% Maybe more details? does the host matter?

\subsection{Implementation.} We implement all algorithms with the newest version of the Cerebras SDK 1.0~\cite{Cerebras-SDK} and runtime. For our Auto-Gen reduce, we compute the necessary parameters in Python. Based on that we generate the source code for each PE. Note that we provide our own (equivalent) implementation of Chain Reduce instead of the one provided in the SDK. A library call would cause reconfiguration of the routers which would yield artificially slow results. 

When implementing collectives for the CS-2 it is important to limit the number of colors as there are only 24 of them. Our 1D implementations utilize up to 3 colors, while the 2D implementations use up to 5. When using our collectives, the rest of the colors would be available to the application. 
%
The routing for the CS-2 is requires avoiding race conditions. Having two wavelets arrive at a router on the same color in the same cycle leads to undefined behaviour. To avoid this, we configure the routers such that at a given cycle they accept wavelets only from a single direction. We do this using control wavelets which alter the routing configuration at runtime.

% Comparing against library
%Additionally, note that we use our implementation of Chain reduce rather than the one in the library, because we are interested in comparing algorithmic approaches. However, note that our prediction of Chain reduce can also be shown to be a hardware lower bound, hence the library implementation cannot perform better than that. This means that the speedups and insights we gain should be at least as good compared to the library version.
%
%Additionally, because we are also interested in capturing relative performance, we implement all collectives in a similar way. This is why we do not use chain reduce from the Cerebras library. However, under the assumption that $T_R \geq 2$~\cite{leighton_fft, DBLP:journals/corr/cerebras_monte_carlo}, the plotted predicted performance for the chain reduce is also the hardware lower bound. The library implementation would not be able to achieve better performance, hence the comparison seems fair.

\subsection{Time Measurements}
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_broadcast_fix.pdf}
        \caption{Broadcast}
        \label{fig:broadcast_fix}
    \end{subfigure}
    % add \hspace if needed
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_reduce_fix.pdf}
        \caption{Reduce}
        \label{fig:reduce_fix}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_allreduce_fix.pdf}
        \caption{AllReduce}
        \label{fig:allreduce_fix}
    \end{subfigure}
    \vspace{-1.5em}
    \caption{Benchmarks for 1D row of 512x1 PEs and increasing vector length.}
    \vspace{0.5em}
    \label{fig:1d_fix}
\end{figure*}


% General
Time measurements in distributed systems have been extensively studied~\cite{hoefler-collmea-sync, collective_benchmarking} and pose challenges, such as lack of a shared clock. A proper measurement methodology is particularly important for the sub-microsecond runtimes we observe. For broadcast, the methodology is easier because the computation starts from a single root, which synchronizes the start time. However, for Reduce we need to synchronize the clocks and ensure that each processor starts at the same time. For all measurements, we start by performing a Reduce to the PE at position $(0,0)$. This constitutes a barrier and ensures that all processes have no other ongoing computations.

% Broadcast
To measure 1D broadcast performance, we use a ping-pong like approach. We execute a broadcast from the leftmost PE, then from the rightmost PE. We repeat this procedure $k$ times and report the end clock time - start clock time at the leftmost PE divided by $2k$. %In our experiments, we use $k=5$.

% Reduce and allreduce
For Reduce and AllReduce we need a different approach, because the execution might start at multiple PEs. Hence, we need to ensure that all PEs start execution at the same time. We perform several calibration runs until a synchronized clock tells us that all PEs start at roughly the same time. The calibration adjusts a so-called \emph{wait parameter} $\alpha$ until the condition is satisfied. Initially, $\alpha=1$.

First, the PE at position $(0,0)$ performs a broadcast that triggers each PE at position $(i,j)$ to sample its local reference clock, called $T_R(i,j)$. Now, each PE $(i, j)$ executes $\alpha(M + N - i - j)$ writes to an empty memory location. After that, each PE samples the start clock $T_S(i,j)$, performs the collective and samples the end clock $T_E(i,j)$. For each PE we calibrate the start and end clock as follows:
\begin{align*}
T_S(i,j)' &= T_S(i,j) - (T_R(i,j) + (i + j + 2)) \\
T_E(i,j)' &= T_E(i,j) - (T_R(i,j) + (i + j + 2))
\end{align*}
This accounts for the difference in time when a PE samples the reference clock, which is $i+j+2$ for a PE at position $(i, j)$ as we use a broadcast to initiate the sampling. %on the distance from the root of the broadcast.
% 
We adjust the wait parameter $\alpha$ and repeat the calibration until the difference in calibrated start times $\max_{i, j} T_S(i,j)' - \min_{i, j} T_S(i, j)'$ is small enough. We obtain a start difference below $57$ cycles for 1D and $129$ cycles for 2D Then, the final measurement is $\max_{i, j} T_E(i, j)' - \min_{i, j} T_S(i, j)'$. This methodology ensures accurate measurements in the wafer-scale setting. In an ideal system $\alpha = 1$ would make all PEs start at the same time since each write takes 1 cycle. However, in order to prevent the PE from overheating, the machine will start inserting no-ops, which we need to adjust for.


\subsection{1D Broadcast}



\textbf{Scaling Vector Length.}
Figure \ref{fig:broadcast_fix} shows the broadcast results for 512 PEs and increasing vector length. As expected, for small vector lengths the runtime is dominated by the distance. Hence, the runtime only grows slowly with the vector length. For vector lengths larger than $512$ bytes, the runtime grows roughly linearly with the vector length. The model matches the predictions closely, with a relative error of at most 21\%.

\textbf{Scaling PE count.}
\Cref{fig:broadcast_inc} shows the results for fixed vector length of 1 KB and increasing number of PEs. Our model predicts the correct trend, with a large initial runtime that accounts for sending the message (contention or energy term) and a gradually increasing contribution of the distance term. The relative error of the prediction is 8\%-21\%.


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_broadcast_inc.pdf}
        \caption{Broadcast}
        \label{fig:broadcast_inc}
    \end{subfigure}
    % add \hspace if needed
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_reduce_inc.pdf}
        \caption{Reduce}
        \label{fig:reduce_inc}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_allreduce_inc.pdf}
        \caption{AllReduce}
        \label{fig:allreduce_inc}
    \end{subfigure}
    \vspace{-0.5em}
    % repeat for other plots, adjust for new lines with \vspace if needed
    \caption{Benchmarks for fixed vector length of 1 KB and increasing number of PEs.}
    %\vspace{0.5em}
    \label{fig:1d_inc}
\end{figure*}

%For increasing vector length our model's predictions have a relative error of up to $95\%$ with an of $91\%$. For increasing number of PEs, we do see that the minimum relative error is $81\%$, corresponding to a difference of only $61$ cycles.

\subsection{1D Reduce}




\textbf{Scaling Vector Length.}
We evaluate Reduce for 512 PEs with increasing vector length in~\Cref{fig:reduce_fix}. As predicted, among the fixed implementations, low depth patterns like the tree excel for small vector lengths, while those with greater depth, like the chain pattern, show inferior performance. 
With increasing vector lengths, energy and contention begin to outweigh depth in impact, resulting in the Two-Phase pattern outperforming others. Finally, for the largest vectors, the contention dominates the runtime and the chain pattern performs best.

% Star
The only exception to the above mentioned predictions is the star pattern. It performs worse than predicted in this scenario. This is likely because of the overhead associated when a PE starts receiving from another PE.  Because the star pattern receives elements from all PEs, this is much more pronounced than for other implementations, especially for large number of PEs. Except for scalars, our experiments and model both suggest that other low-depth patters, such as Tree or our Two-Phase algorithm, are faster.
%We hypothesize that this is an implementation or SDK issue. We observe an overhead whenever a PE starts receiving from another PE. Because the star pattern receives elements from all PEs, this is much more pronounced than for other implementations, especially for large number of PEs. Our model allows us to estimate the potential benefit of a tuned implementation~\cite{massively_scalable_stencil_cerebras}. We conclude that except for scalars, other low-depth patterns are faster. %However, note that our prediction is the lower bound for any implementation of the approach

%Right now in the implementation, there is an overhead when we start receiving vectors from another PE. Because the star pattern receives elements from all PEs, this is much more pronounced than for other implementations, however, since what we plot for the star pattern is essentially contention, it is also the lower bound for its performance. Therefore, we know it would not perform better than other patterns except when reducing a scalar. For the scalar Reduce, we know from~\cite{massively_scalable_stencil_cerebras} that implementation which achieves our predictions for scalars is possible. However, the given implementation has been done in a stack only available for people from Cerebras. On the other hand by seeing that the measured performance is far from the predictions, we could deduce that the code should be further optimized.


% Pre Order
Overall, our Auto-Gen Reduce is the fastest pattern except when reducing a scalar. There, it is slower by at most $110$ cycles. It outperforms the chain pattern, based on the current library implementation, by up to $3.16$x. This further confirms the choice of our model as a tool for automatic performance tuning.

% Performance Trends
With mean relative error per pattern ranging from $12\%$ to $35\%$, the general performance trends are well captured by our model. When choosing two different patterns, our model is able to very accurately predict which of the two performs best for the given vector length and number of PEs. In the cases where it mispredicts, the difference is at most $114$ cycles. This means that, even if the model's predictions are not perfect, the chosen algorithm remains highly competitive and close to the best possible performance.

\textbf{Scaling PE count.}
% Increasing number of PEs
 Additionally, we evaluate the Reduce operation for a fixed vector length of 1 KB across an increasing number of PEs, as illustrated in \Cref{fig:reduce_inc}. Our model correctly predicts that initially the chain pattern performs best because with very few PEs, contention has a larger impact than the depth. With increasing number of PEs, the depth becomes more significant, and, as expected, the two phase pattern performs better. 

% Remarks, relative to the fix PEs
Just as for the results with the fixed number of PEs, we see that our Auto-Gen Reduce implementation is the fastest throughout. Two-Phase offers similar performance as Auto-Gen for $64$ or more PEs. Interestingly, predictions for the star pattern have high accuracy, with a $10\%$ minimum relative error. This is likely because the runtime is dominated by the vector length rather than the number of PEs in this case. Overall, our model predicts performance trends accurately, with a mean relative error between $13\%$ and $28\%$. 





\subsection{1D AllReduce}




% fix allreduce, reduce-then-broadcast
\textbf{Scaling Vector Length.} We evaluate AllReduce for 512 PEs and increasing vector length, see Figure~\ref{fig:allreduce_fix}. As expected, for the reduce-then-broadcast AllReduce implementations the runtime increases by the cost of performing a broadcast with respect to the corresponding Reduce variant. We can draw the same insights as from the Reduce results, e.g., how the optimal pattern changes based on the vector length. Our Auto-Gen AllReduce gains a $2.47$x improvement over the chain-then-broadcast approach, which the current library is based on. Additionally, just like for Reduce, our model accurately predicts performance trends and which pattern will perform best.

% Ring
We also plotted predicted performance for ring pattern. We have already observed that our model accurately predicts which algorithm performs best. Even accounting for a $15\%$ prediction error, the largest observed overall, the ring algorithm is never be the best choice. Hence, we refrain from providing an implementation. This underscores the utility of our model is saving engineering effort on sub-optimal and unpromising approaches. Moreover, we see that algorithms designed for the traditional distributed memory setting do not translate well into the wafer-scale setting, where it is important to leverage multicasting and pipelining.

%This leads us to believe that performance gain from either ring would be negligible. This observation underscores the need for algorithms specifically tailored for the WSE in mind, leveraging hardware features such as multicast.

% inc PE
\textbf{Scaling PE count.} Moreover, we evaluate AllReduce for a fixed vector length of 1 KB and increasing number of PEs, see \Cref{fig:allreduce_inc}. Again, for the reduce-then-broadcast implementations, we observe similar results as for Reduce. We see that for 4 PEs, the predicted ring performance is a bit better than the chain AllReduce. However, the expected performance gain is not significant. For numbers of PEs larger than $8$, we see that the reduce-then-broadcast implementations would perform significantly better than the ring, outperforming it by possibly even $1.4$x. This further shows how powerful the multicast feature for the CS-2 is.

\subsection{2D Collectives}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_reduce_2d_fix.pdf}
        \caption{2D Reduce for $512\times 512$ PEs.}
        \label{fig:experiments-2d-reduce-fix}
    \end{subfigure}
    % add \hspace if needed
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_allreduce_2d_fix.pdf}
        \caption{2D AllReduce for $512\times 512$ PEs.}
        \label{fig:experiments-2d-allreduce-fix}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/plot_reduce_2d_inc.pdf}
        \caption{2D Reduce for vector length of 1KB.}
        \label{fig:experiments-2d-reduce-inc}
    \end{subfigure}
    \vspace{-1.5em}
    \caption{2D Reduce and AllReduce benchmarks.}
    \vspace{1em}
    \label{fig:experimental_plots_2d}
\end{figure*}



\textbf{Scaling Vector Length.} We also evaluate our implementations on the full chip of $512\times512$ PEs and increasing vector length. For Reduce, the results can be found in Figure~\ref{fig:experiments-2d-reduce-fix}. The performance trends are as predicted. They are similar to to 1D setting. Our X-Y Auto-Gen Reduce outperforms the X-Y Chain by up to $3.27 \times$.

% Snake
The predictions for the snake pattern are at most $10\%$ off. As expected, it performs very poorly. This is because of its linear depth in the number of PEs, which is over 200'000 for this experiment. Interestingly, these results indicate that $T_R = 2$ on average. Any other choice of $T_R$ would lead to significantly worse predictions.

% Accuracy
Moreover, we have a relative error that is very similar to what we were seeing for 1D. The predictions are slightly worse because when we execute X-Y Reduce, after reducing on the X-axis, we need to load some values into registers which adds additional overhead. Again, our model is able to predict very well which pattern will perform best for a given vector length.

% 2D AllReduce benchmark
Figure~\ref{fig:experiments-2d-allreduce-fix} shows the  2D AllReduce results for fixed number of PEs and increasing vector length. %We have the similar insights and trends as for reduce. 
The relative error of our predictions remains almost the same. Moreover, our X-Y Auto-Gen AllReduce implementation outperforms the X-Y Auto-Gen AllReduce implementation by up to $2.54 \times$.

\textbf{Scaling PE count.} Just like for 1D benchmarks, we measure performance for fixed vector length and increasing 2D grid of PEs from $4\times4$ to $512\times512$. The results can be found in Figure~\ref{fig:experiments-2d-reduce-inc}. As expected, when we have few PEs and we are bandwidth bound, the Snake pattern performs best. Then as the number of PEs grows, the X-Y Chain and finally the X-Y Two Phase pattern are best. 

% Auto-Gen
Our X-Y Auto-Gen reduce once again achieves good overall performance across the board. The only exception is for $4\times 4$ PEs, where the Snake is better. This demonstrates that generating code based on our model works well both in the 1D and 2D setting.



==> sections/allgather.tex <==
\section{Allgather}
DISCUSS and TODO: I had an idea for an allgather implementation, for which we could show that it is hardware optimal for even number of PEs and for odd number of PEs it would be worse by about $2T_R + 1$. Either way, I think we would then use it in the chain allreduce.

In an allgather with $P$ PEs and each with a vector of length $B$, each PE needs to receive $B(P - 1)$ wavelets. The time before a PE can receive the first wavelet is $2T_R + 1$. Because a PE can then receive at most one wavelet per cycle, the lower bound for allgather is $B(P - 1) + 2T_R$ cycles.

==> sections/analysis.tex <==
\section{Theoretical Analysis}

We  derive the cost of a common messaging primitive, the \textsc{Visit}, which will underly all our cost analysis. It sends $B$ values from a processor $p$ to a processor $p'$ that is at Hamming distance $P-1$ from $p$. Along the way of the shortest path, the values are sent through $V$ intermediate stops. That is, the $B$ values travel through $V+2$ processors $p, p_0, \dotsc  p_V, p'$ overall. 
\begin{lemma}
The number of cycles $T_{\textsc{Visit}}$ of the \textsc{Visit} for $P$ PEs, vector size $B$ and $V$ intermediate stops is
\begin{align}
T_{\textsc{Visit}}(P, B, V) = B + P - 1  + (2 T_R + 1) (V + 1) \enspace .
\end{align}   
\end{lemma}
\begin{proof}
The depth is $D=V+1$, the distance is $L=P-1$, the energy is $(P-1)B$, and the contention is $B$.
\end{proof}

\paragraph{Chain Reduce}


\paragraph{Tree Reduce}
For a 1D tree reduce on $P$ processors, the depth is $\log_2 P$, the distance is $P-1$, the energy is $\frac{B}{2} (P-1)\log_2 P$, and the contention is $B\log_2(P)$ Hence, we get the estimate for the number of cycles of a tree reduce $T_{\textsc{Tree}}$ of 
\begin{align}
T_{\textsc{Tree}} = P - 1 + (2 T_R + 1) \log_2 P + \frac{B}{2} \log_2 P \enspace 
\end{align}
We can see that for large vector sizes $B$, the cost is dominated by the energy term (which captures congestion), whereas for small vector sizes, it is dominated by the distance and depth terms.


\paragraph{2 Phase Reduce}

The depth is $S + \lceil \frac{P}{S} \rceil$, the distance is $P-1$, and  the energy is $(S-1) \lceil \frac{P}{S} \rceil B + (P - S) B$. Assuming $S$ divides $P$, we estimate
\begin{align}
T_{\textsc{2phase}} = P - 1 + (2 T_R + 1) \left(S + \frac{P}{S} \right) + 2B - \frac{S}{P-1} B
\end{align}

\paragraph{Scalar Reduce}

The depth is $1$, the energy is $B \frac{P(P-1)}{2}$, and the distance is $P-1$. 

\begin{align}
T_{\textsc{scalar}} = P + 2 T_R + \frac{B P}{2}
\end{align}
% Note: This under-estimates the runtime by a factor of 2 for large P.

==> sections/gemm.tex <==
% \section{GEMM}\label{sec:gemm}
% DISCUSS: Should we include it? Is there even enough space?
